Robust Discrete-Time Pontryagin Maximum Principle on Matrix Lie Groups

This article considers a discrete-time robust optimal control problem on matrix Lie groups. The underlying system is assumed to be perturbed by exogenous unmeasured bounded disturbances, and the control problem is posed as a min-max optimal control wherein the disturbance is the adversary and tries to maximise a cost that the control tries to minimise. Assuming the existence of a saddle point in the problem, we present a version of the Pontryagin maximum principle (PMP) that encapsulates first-order necessary conditions that the optimal control and disturbance trajectories must satisfy. This PMP features a saddle point condition on the Hamiltonian and a set of backward difference equations for the adjoint dynamics. We also present a special case of our result on Euclidean spaces. We conclude with applying the PMP to robust version of single axis rotation of a rigid body.

==> introduction-ext.tex <==
\section{Introduction}

%Optimal control. PMP. Discrete optimal control. MPC, PMP. 

%Robust control. Robust optimal control. 

%Control for certain systems - Geometric control. Geometric optimal control. Discrete geometric optimal control.  

Optimal control is a cornerstone in the theory of modern control \cite{agrachev,liberzon}.
%{\cg check karmvir's references, liberzon's references, google for a survey paper}. 
%Apart from theoretical work of a more fundamental nature which combine optimal control with areas like mathematical theory of dynamical systems \cite{agrachev-2003} and analytical mechanics \cite{bloch-1999}, it has also been applied to various practical problems in physics and engineering, like mechanical systems \cite{gibson-1985,bloch-2008}, aerospace engineering \cite{ben-asher} \cite{trelat-2003,trelat-2012} bio-engineering \cite{moreno-1999}, in the theory of observers \cite{mahony-2012,trelat-2013} and quantum mechanics \cite{khaneja-2001}. 
The Pontryagin maximum principle \cite{pontryagin} (henceforth referred to as the PMP) constitutes an integral part of optimal control theory, and it provides first order necessary conditions for optimality.
%derived using ideas from calculus of variations, which an optimal control satisfies. 
These necessary conditions make the process of finding an optimal control significantly simpler by narrowing the set of admissible controls into a subset of candidate optimisers, and they are used by numerical algorithms to search for an optimal control. It is, in fact, one of the most widely used tools in optimal control apart from the Hamilton-Jacobi-Bellman (HJB) approach. %The HJB yields sufficient conditions for optimality and requires the solution of a partial differential equation, while the PMP leads to a two point boundary alue problem. Both, the HJB and the PMP can, in general, only be solved numerically, and numerical algorithms for partial differential equations are much more difficult than ones for two point boundary value problems (which contains two ordinary differential equations).
%and in more general settings as well \cite{clarke-1976,sussman-2008}. 
The PMP has traditionally been studied in a continuous-time setting, and while the discrete-time version \cite{bolt} received less attention in the initial stages, there have recently been several investigations into the discrete time PMP, for instance, in the presence of constraints and in the geometric setting; see, e.g., \cite{gupta-2019, mishal-2020,prad-2019,karmvir-2018} and the references therein. %The discrete time version was initially developed under suitable convexity assumptions \cite{hubert-1966,halkin-1966,holt-1966} and has since then been extended into a well formed theory .}
%There have been numerous investigations into the PMP, for instance, %on the geometry behind the problem and the role of abnormal extremals \cite{barbero-2008}, 
%with constraints \cite{dubo-1968,prad-2019}, and in a non-smooth setting \cite{mord-1976,shruti-2019}. 
%The Pontryagin maximum principle has traditionally been studied in a continuous time setting. The discrete time version has received lesser attention. The discrete time version was initially developed under suitable convexity assumptions \cite{hubert-1966,halkin-1966,holt-1966} and has since then been extended into a well formed theory \cite{boltyanskii-1975,bolt}. 


The mathematical model of any engineering system is almost always an approximation of its actual behaviour, and consequently, it is essential to address the robustness aspect of control schemes. By this we mean the ability of the controller to give satisfactory performance under system modelling uncertainties or the presence of exogenous unmeasured disturbances.
%A natural question (that of robust control, to be specific) which arises is that of probing into systems that have uncertainty or are perturbed by external disturbances. 
%In the stochastic framework, the Linear Quadratic Gaussian controller models all system uncertainty and measurement noise as Gaussian signals, and is a robust version of the the Linear Qudratic Regulator. 
Our emphasis here will be on deterministic controllers formulated as min-max optimisation problems (also studied as games), in which the disturbance is the adversary and tries to maximise the cost which the control tries to minimise  \cite{basar-1995,basar-1998,chen-1997,
chern-2005,raimondo-2009}.

%\cite{basar-1995,basar-1998}, \cite{mayne-1997,sharav-1999,
%bemporad-2003,bertsimas-2007},\cite{chern-2005,wu-2013},\cite{chen-1997},\cite{raimondo-2009}. 
%Min max problems have also found their way into observer design  \cite{basar-1991,ravi-1991}.  

PMPs for robust optimal control problems of the aforementioned type have been derived in \cite{vinter-2005} for continuous time systems with uncertainties, and in \cite{bolt-robust} for discrete time systems when the set of (parametric) uncertainties is assumed to be a finite set. For continuous time systems, there has been considerable work in the game theoretic framework on the min-max control for systems with disturbances, we pick the representative articles \cite{bernhard-2015,bressan-2011} from that literature, since they demonstrate results which closely resemble the PMP. When \cite{bressan-2011} is specialized to our setting of a min-max problem, we arrive at a zero sum differential game which has a Nash equilibrium (a game theoretic analog of a saddle point). This gives rise to two distinct sub-problems, one of minimising the cost over allowable controls (and this problem is parametrised by the optimal disturbance) and the other of maximising the cost over allowable disturbances (which is paramerised by the optimal control). They proceed to apply the PMP on both sub-problems individually to arrive at two sets of two-point boundary value problems, each with their own Hamiltonians and covectors, each parametrized by the solution of the other. \cite{bernhard-2015} takes this further by deriving a single maximum principle with a single Hamiltonian and single covector by employing the Isaacs equation in an interesting fashion. Our approach here is derived from the ideas in these two articles, but we operate under a different context and regime that we now explain.
 
A broad class of aerospace and mechanical systems evolve on the class of smooth manifolds known as Lie groups. These state spaces are `nonlinear' and curved, and as such lack a vector space structure. This feature warrants new techniques to be developed in order to study these systems, and such techniques fall under the broad umbrella of geometric mechanics and control \cite{agrachev,marsden}. 
Optimal control of such systems has received significant attention \cite{agrachev,bloch-2015}; in particular, PMPs for systems evolving on smooth manifolds has been studied both in continuous \cite{sussman-1997} and discrete time \cite{chang-2011,gupta-2019,mishal-2020,karmvir-2018} in considerable detail. %In the context of discrete-time systems, \cite{bloch-2010} establishes an analog of Hamilton-Jacobi theory. 
More specifically, geometric discrete-time optimal control, designed specifically to respect the non-flat nature of the underlying state spaces, has been of great interest in the engineering community since the associated techniques eliminate problems that occur by using local parametrisation %\cite{bloch-2006,leon-2007,fernando-2013,karmvir-2018-jgcd}.
\cite{bloch-2006,fernando-2013,karmvir-2018-jgcd}.

In \cite{karmvir-2018}, a discrete-time PMP for optimal control problems for systems evolving on matrix Lie groups was presented. That work however did not consider the performance of the controller under the effect of exogenous unmeasured disturbances. Our work here takes the problem a step further by incorporating the effect of bounded disturbances acting on the class of systems considered in \cite{karmvir-2018} and by posing the optimal control problem as a min-max problem. Assuming the existence of a saddle point of the cost function, we provide first order necessary conditions that the control and disturbance satisfy for optimality are presented in the form of a modification of the PMP. We arrive at a saddle point condition on the Hamiltonian and backward difference equations for the covector (also termed adjoint) dynamics. We also present a specialised version of our result to Euclidean spaces for those interested in directly applying it to such systems.
%We treat a discrete time robust optimal control problem on Lie groups posed as a min-max optimisation problem. We let the control system be perturbed by disturbances which are bounded pointwise in time. 
%Assuming the existence of a saddle point of the cost function, we provide necessary conditions that the control and disturbance satisfy, in the form of a maximum principle, which gives a saddle point condition on the Hamiltonian and backward difference equations for the covector (also termed adjoint) dynamics. 
Our results are similar in spirit to \cite{bernhard-2015} but different in three very significant aspects:
\begin{itemize}[leftmargin=10pt, align=left]
	\item We consider a problem that evolves in discrete-time, for which it is not possible to derive the maximum principle from a min-max version of the Bellman's equation. This is relevant, since in continuous-time the PMP can be derived using ideas from the HJB partial differential equation \cite[Chapter 5]{liberzon}, and similarly the modification of PMP in \cite{bernhard-2015} can be derived using ideas from the Isaacs equation.
	\item \cite{bernhard-2015} hypothesizes that the Hamiltonian satisfies a saddle point condition \emph{before} establishing their result. We do not do make any such assumption, but instead the saddle point condition appears naturally in our development. 
	\item \cite{bernhard-2015} assumes that the abnormal multiplier used in the Hamiltonian is non-zero at the outset, but we \emph{prove} that it must always be non-zero in our setting.
\end{itemize}
The results closest to ours are in \cite{bolt-robust}, but as noted earlier, \cite{bolt-robust} considers parametric uncertainty in the system where the parameter set is assumed to be finite.

This paper is organized as follows. 
Section \ref{sec:prelim} contains preliminaries and the statement of the maximum principle for our case, which is proven in Section \ref{sec:proof}.
Section \ref{sec:example} contains an aerospace example where our theory is applied.

%Geometric optimal control {\cg chang - proof of PMP on manifolds,}

